Proactive AI: From Turns to Replannable Dialogue Timelines

Conventional large-language-model chat interfaces typically follow user-initiated turns: each request elicits a response, after which the system waits for further input. Human asynchronous communication instead unfolds over time through message bursts, delays, silence, resumed topics, and self-initiated contact. Proactive dialogue therefore requires not only deciding when to speak, but also managing pending conversational actions and allowing them to be revised as context evolves. We introduce Proactive AI, a framework for proactive dialogue built around replannable temporal message queues. The framework treats interaction as a continuous event timeline and unsent conversational actions as revisable state. A user event, dialogue-pacemaker event, or scheduled decision may yield silence, one or more immediate messages, or future conversational actions. The system may also observe a user message without an immediate visible response and defer the response decision. Before delivery, every planned message must be reconsidered against the current context; reaching a scheduled time does not itself authorize delivery. We provide a formal semantics that characterizes when future conversational actions may be revised, withdrawn, or executed as context evolves. The framework extends AI participation beyond responses to current requests, enabling self-initiated exchanges without new requests, sustained follow-up over time, and revisions of subsequent actions as context evolves. It provides an executable basis for long-term human-AI interaction in tutoring, scientific collaboration, and everyday companionship.

==> figures/conversation-examples.tex <==
\begin{tikzpicture}[pai-figure]

% (a) A familiar chat interface constrained to paired turns.
\filldraw[pai-panel]
  (0,0.10) rectangle (5.10,5.70);
\node[pai-panel-title, anchor=west] at (0.25,5.42)
  {a\quad Paired request--response};
\filldraw[pai-chat-surface]
  (0.18,0.28) rectangle (4.92,5.13);

\node[pai-secondary] at (2.55,4.81) {09:00};
\node[pai-user-avatar] at (4.48,4.31) {U};
\node[pai-user-message, anchor=east, text width=2.15cm] at (4.12,4.31)
  {Help me prepare.};
\node[pai-agent-avatar] at (0.63,3.57) {AI};
\node[pai-agent-message, anchor=west, text width=2.15cm] at (0.98,3.57)
  {Here is a plan.};

\draw[pai-divider]
  (0.68,3.00) -- (4.42,3.00);
\node[pai-secondary] at (2.55,2.75) {09:05};
\node[pai-user-avatar] at (4.48,2.23) {U};
\node[pai-user-message, anchor=east, text width=1.70cm] at (4.12,2.23)
  {What next?};
\node[pai-agent-avatar] at (0.63,1.47) {AI};
\node[pai-agent-message, anchor=west, text width=3.05cm] at (0.98,1.47)
  {Try a mock interview.};
\node[pai-secondary] at (2.55,0.75)
  {one prompt $\rightarrow$ one answer};

% (b) A concrete failure in which a scheduled message becomes stale.
\filldraw[pai-panel]
  (5.35,0.10) rectangle (15.90,5.70);
\node[pai-panel-title, anchor=west] at (5.60,5.42)
  {b\quad A stale scheduled message};
\filldraw[pai-chat-surface]
  (5.53,0.28) rectangle (15.72,5.13);

\node[pai-secondary] at (10.62,4.87) {Mon 09:00};
\node[pai-user-avatar] at (15.20,4.41) {U};
\node[pai-user-message, anchor=east, text width=2.45cm] at (14.82,4.41)
  {Interview tomorrow.};
\node[pai-user-avatar] at (15.20,3.87) {U};
\node[pai-user-message, anchor=east, text width=1.75cm] at (14.82,3.87)
  {I'm nervous.};
\node[pai-agent-avatar] at (6.05,3.27) {AI};
\node[pai-agent-message, anchor=west, text width=2.55cm] at (6.40,3.27)
  {That makes sense.};
\node[pai-agent-avatar] at (6.05,2.73) {AI};
\node[pai-agent-message, anchor=west, text width=2.55cm] at (6.40,2.73)
  {Want to rehearse?};

\node[pai-secondary] at (10.62,2.23) {Mon 16:30};
\node[pai-user-avatar] at (15.20,1.79) {U};
\node[pai-user-message, anchor=east, text width=2.45cm] at (14.82,1.79)
  {Interview cancelled.};
\draw[pai-silence-span]
  (8.90,1.30) -- (12.34,1.30);
\node[pai-secondary, fill=white, inner xsep=4pt] at (10.62,1.30)
  {plan remains unchanged overnight};
\node[pai-agent-avatar] at (6.05,0.61) {AI};
\node[pai-agent-message, anchor=west, text width=4.65cm] at (6.40,0.61)
  {Good luck with your interview today!};

\end{tikzpicture}


==> figures/interaction-timelines.tex <==
\begin{tikzpicture}[pai-figure]

% (c) Conventional request-response turns.
\filldraw[pai-panel]
  (0,5.02) rectangle (15.9,7.25);
\node[pai-panel-title, anchor=west] at (0.28,6.92) {c};
\node[pai-panel-title, anchor=east] at (1.42,6.45) {$U$};
\node[pai-panel-title, anchor=east] at (1.42,5.70) {$AI$};
\draw[pai-axis] (1.72,5.30) -- (15.50,5.30) node[above left=-1pt] {$t$};

\node[pai-user-event] (a-u1) at (3.00,6.45) {$u_1$};
\node[pai-agent-event] (a-a1) at (4.70,5.70) {$a_1$};
\node[pai-user-event] (a-u2) at (7.20,6.45) {$u_2$};
\node[pai-agent-event] (a-a2) at (8.90,5.70) {$a_2$};
\node[pai-user-event] (a-u3) at (11.40,6.45) {$u_3$};
\node[pai-agent-event] (a-a3) at (13.10,5.70) {$a_3$};
\foreach \n in {a-u1,a-a1,a-u2,a-a2,a-u3,a-a3} {
  \draw[pai-event-line] (\n.south) -- (\n.south |- 0,5.30);
}
\draw[pai-causal] (a-u1.south east) to[out=-28,in=145] (a-a1.north west);
\draw[pai-causal] (a-u2.south east) to[out=-28,in=145] (a-a2.north west);
\draw[pai-causal] (a-u3.south east) to[out=-28,in=145] (a-a3.north west);

% (d) Human asynchronous messaging.
\filldraw[pai-panel]
  (0,2.52) rectangle (15.9,4.75);
\node[pai-panel-title, anchor=west] at (0.28,4.42) {d};
\node[pai-panel-title, anchor=east] at (1.42,3.95) {$P_A$};
\node[pai-panel-title, anchor=east] at (1.42,3.20) {$P_B$};
\draw[pai-axis] (1.72,2.80) -- (15.50,2.80) node[above left=-1pt] {$t$};

\node[pai-user-event] (b-m1) at (2.75,3.95) {$m_1$};
\node[pai-user-event] (b-m2) at (3.75,3.95) {$m_2$};
\node[pai-agent-event] (b-r1) at (5.65,3.20) {$r_1$};
\node[pai-agent-event] (b-r2) at (6.65,3.20) {$r_2$};
\node[pai-user-event] (b-m3) at (8.45,3.95) {$m_3$};
\node[pai-agent-event] (b-r3) at (10.20,3.20) {$r_3$};
\node[pai-agent-event] (b-i1) at (13.35,3.20) {$i_1$};
\foreach \n in {b-m1,b-m2,b-r1,b-r2,b-m3,b-r3,b-i1} {
  \draw[pai-event-line] (\n.south) -- (\n.south |- 0,2.80);
}
\draw[pai-silence-span]
  (10.80,3.57) -- node[above, inner sep=2pt] {$\Delta t$} (12.75,3.57);

% (e) Replannable proactive AI timeline.
\filldraw[pai-panel]
  (0,0.02) rectangle (15.9,2.25);
\node[pai-panel-title, anchor=west] at (0.28,1.92) {e};
\node[pai-panel-title, anchor=east] at (1.42,1.45) {$U$};
\node[pai-panel-title, anchor=east] at (1.42,0.70) {$AI$};
\draw[pai-axis] (1.72,0.30) -- (15.50,0.30) node[above left=-1pt] {$t$};

\filldraw[pai-plan-group]
  (4.82,0.42) rectangle (10.02,1.14);
\node[pai-secondary, text=paiDecision, fill=paiDecisionLight,
  anchor=west, inner xsep=2pt] at (4.96,1.14) {one plan};

\node[pai-user-event] (c-u1) at (2.35,1.45) {$u_1$};
\node[pai-user-event] (c-u2) at (3.25,1.45) {$u_2$};
\node[pai-decision] (c-plan) at (4.22,0.70) {$\pi$};
\node[pai-agent-event] (c-a1) at (5.52,0.70) {$a_1$};
\node[pai-agent-event] (c-a2) at (6.92,0.70) {$a_2$};
\node[pai-user-event] (c-u3) at (8.18,1.45) {$u_3$};
\node[pai-pending-event] (c-pending) at (9.48,0.70) {$\widehat{a}_3$};
\node[pai-decision] (c-delta) at (11.62,0.70) {$\delta$};
\node[pai-agent-event] (c-a4) at (13.30,1.05) {$a_4$};
\node[draw=paiNeutral, circle, minimum size=0.44cm, inner sep=0pt]
  (c-silence) at (13.30,0.58) {$\varnothing$};
\foreach \n in {c-u1,c-u2,c-plan,c-a1,c-a2,c-u3,c-pending,c-delta,c-silence} {
  \draw[pai-event-line] (\n.south) -- (\n.south |- 0,0.30);
}
\draw[pai-event-line] (c-a4.south) -- (c-a4.south |- 0,0.30);
\draw[pai-causal] (c-u1.south east) to[out=-25,in=155] (c-plan.north west);
\draw[pai-causal] (c-u2.south east) to[out=-35,in=135] (c-plan.north west);
\draw[pai-causal] (c-plan.east) -- (c-a1.west);
\draw[pai-silence-span]
  (c-a1.east) -- node[pai-secondary, fill=paiDecisionLight,
  inner xsep=2pt, above=1pt] {$\Delta_1$} (c-a2.west);
\draw[pai-silence-span]
  (c-a2.east) -- node[pos=0.25, pai-secondary, fill=paiDecisionLight,
  inner xsep=2pt, above=1pt] {$\Delta_2$} (c-pending.west);
\draw[pai-revision] (c-u3.south east) to[out=-25,in=145] (c-pending.north west);
\node[pai-cancel-mark]
  at (c-pending.north east) {$\times$};
\draw[pai-causal] (c-delta.east) -- (12.35,0.70);
\draw[pai-causal] (12.35,0.70) -- (c-a4.west);
\draw[pai-causal] (12.35,0.70) -- (c-silence.west);

\end{tikzpicture}

